The Hubble constant anchor galaxy NGC 4258: metallicity and distance from blue supergiants

A quantitative spectroscopic study of blue supergiant stars in the Hubble constant anchor galaxy NGC 4258 is presented. The non-LTE analysis of Keck I telescope LRIS spectra yields a central logarithmic metallicity (in units of the solar value) of [Z] = -0.05\pm0.05 and a very shallow gradient of -(0.09\pm0.11)r/r25 with respect to galactocentric distance in units of the isophotal radius. Good agreement with the mass-metallicity relationship of star forming galaxies based on stellar absorption line studies is found. A comparison with HII region oxygen abundances obtained from the analysis of strong emission lines shows reasonable agreement when the Pettini & Pagel (2004) calibration is used, while the Zaritsky et al. (1994) calibration yields values that are 0.2 to 0.3 dex larger. These results allow to put the metallicity calibration of the Cepheid Period--Luminosity relation in this anchor galaxy on a purely stellar basis. Interstellar reddening and extinction are determined using HST and JWST photometry. Based on extinction-corrected magnitudes, combined with the stellar effective temperatures and gravities we determine, we use the Flux-weighted Gravity--Luminosity Relationship (FGLR) to estimate an independent spectroscopic distance. We obtain a distance modulus m-M = 29.38\pm0.12 mag, in agreement with the geometrical distance derived from the analysis of the water maser orbits in the galaxy's central circumnuclear disk.

==> Table2_old.tex <==
03 & $21.411\pm0.020$ & $21.439\pm0.020$ & \nodata          & $21.540\pm0.020$ & $21.864\pm0.032$ \\[-0.4ex]
04 & $21.284\pm0.020$ & $21.282\pm0.020$ & \nodata          & $21.233\pm0.020$ & $20.788\pm0.054$ \\[-0.4ex]
05 & $21.904\pm0.020$ & $21.866\pm0.015$ & $21.880\pm0.032$ & $21.949\pm0.026$ & $21.934\pm0.048$ \\[-0.4ex]
06 & $21.453\pm0.020$ & $21.294\pm0.015$ & \nodata          & $21.109\pm0.015$ & $20.210\pm0.031$ \\[-0.4ex]
08 & $21.526\pm0.023$ & $21.391\pm0.018$ & $21.368\pm0.034$ & $21.157\pm0.021$ & $21.135\pm0.095$ \\[-0.4ex]
10 & $22.271\pm0.020$ & $22.165\pm0.015$ & \nodata          & $21.934\pm0.015$ & $21.851\pm0.134$ \\[-0.4ex]
11 & $21.704\pm0.020$ & $21.659\pm0.015$ & \nodata          & $21.549\pm0.017$ & $21.608\pm0.054$ \\[-0.4ex]
12 & $21.245\pm0.020$ & $20.896\pm0.015$ & \nodata          & $19.836\pm0.015$ & $18.147\pm0.049$ \\[-0.4ex]
13 & $21.885\pm0.020$ & $21.881\pm0.015$ & \nodata          & $21.841\pm0.015$ & $21.794\pm0.087$ \\[-0.4ex]
14 & $21.932\pm0.020$ & $21.813\pm0.015$ & $21.716\pm0.025$ & $21.520\pm0.015$ & $21.057\pm0.108$ \\[-0.4ex]
16 & $21.597\pm0.022$ & $21.501\pm0.015$ & $21.476\pm0.025$ & $21.443\pm0.015$ & $21.407\pm0.047$ \\[-0.4ex]
17 & $22.070\pm0.030$ & $22.033\pm0.028$ & \nodata          & $21.947\pm0.036$ & $22.396\pm0.063$ \\[-0.4ex]
20 & $21.650\pm0.020$ & $21.252\pm0.015$ & \nodata          & $20.724\pm0.015$ & $20.157\pm0.073$ \\[-0.4ex]
21 & $22.129\pm0.020$ & $22.044\pm0.015$ & $22.199\pm0.025$ & $21.852\pm0.015$ & $21.719\pm0.128$ \\[-0.4ex]
23 & $21.591\pm0.024$ & $21.044\pm0.015$ & $20.849\pm0.025$ & $20.390\pm0.015$ & $20.081\pm0.068$ \\[-0.4ex]
26 & $21.487\pm0.020$ & $21.140\pm0.015$ & $20.964\pm0.025$ & $20.700\pm0.015$ & $20.453\pm0.070$ \\[-0.4ex]
29 & $20.849\pm0.020$ & $20.584\pm0.015$ & $20.483\pm0.037$ & $20.098\pm0.015$ & $19.952\pm0.049$ \\[-0.4ex]
31 & $22.034\pm0.020$ & $22.093\pm0.015$ & $22.113\pm0.025$ & $22.036\pm0.020$ & $22.318\pm0.050$ \\[-0.4ex]
32 & $21.419\pm0.020$ & $21.373\pm0.020$ & $21.363\pm0.025$ & $21.267\pm0.015$ & $21.548\pm0.037$ \\[-0.4ex]
33 & $21.882\pm0.035$ & $21.832\pm0.015$ & \nodata          & $21.706\pm0.016$ & $21.587\pm0.085$ \\[-0.4ex]


==> Table3_old.tex <==
01 & 21.509$\pm0.004$ & 21.499$\pm0.003$ & 21.506$\pm0.004$ & 21.455$\pm0.004$ & 21.338$\pm0.005$ & 21.297$\pm0.007$ \\[-0.4ex]
08 & 21.318$\pm0.003$ & 21.094$\pm0.003$ & 21.046$\pm0.003$ & 20.992$\pm0.004$ & 20.854$\pm0.006$ & 20.801$\pm0.007$ \\[-0.4ex]
09 & 22.667$\pm0.010$ & 21.865$\pm0.006$ & 21.202$\pm0.005$ & 20.521$\pm0.003$ & 20.057$\pm0.005$ & 19.771$\pm0.007$ \\[-0.4ex]
11 & 21.630$\pm0.004$ & 21.596$\pm0.004$ & 21.650$\pm0.005$ & 21.673$\pm0.006$ & 21.643$\pm0.014$ & 21.864$\pm0.027$ \\[-0.4ex]
13 & 21.715$\pm0.004$ & 21.653$\pm0.004$ & 21.681$\pm0.006$ & 21.664$\pm0.007$ & 21.497$\pm0.015$ & 21.496$\pm0.022$ \\[-0.4ex]
14 & 21.597$\pm0.004$ & 21.508$\pm0.004$ & 21.415$\pm0.004$ & 21.296$\pm0.003$ & 21.187$\pm0.005$ & 21.127$\pm0.007$ \\[-0.4ex]
16 & 21.499$\pm0.004$ & 21.560$\pm0.004$ & 21.533$\pm0.004$ & 21.497$\pm0.005$ & 21.490$\pm0.009$ & 21.544$\pm0.015$ \\[-0.4ex]
18 & 20.444$\pm0.002$ & 20.364$\pm0.003$ & 20.368$\pm0.005$ & 20.328$\pm0.007$ & 20.092$\pm0.017$ & 19.778$\pm0.021$ \\[-0.4ex]
22 & 21.495$\pm0.004$ & 20.728$\pm0.002$ & 20.009$\pm0.002$ & 19.261$\pm0.002$ & 18.552$\pm0.002$ & 18.257$\pm0.002$ \\[-0.4ex]
23 & 20.614$\pm0.002$ & 20.260$\pm0.002$ & 20.108$\pm0.002$ & 19.972$\pm0.003$ & 19.695$\pm0.004$ & 19.610$\pm0.006$ \\[-0.4ex]
24 & 20.617$\pm0.003$ & 20.374$\pm0.002$ & 20.304$\pm0.002$ & 20.219$\pm0.003$ & 20.025$\pm0.006$ & 20.011$\pm0.008$ \\[-0.4ex]
27 & 20.434$\pm0.003$ & 20.314$\pm0.003$ & 20.107$\pm0.003$ & 19.860$\pm0.002$ & 19.328$\pm0.002$ & 19.108$\pm0.003$ \\[-0.4ex]
29 & 20.353$\pm0.003$ & 20.109$\pm0.002$ & 20.009$\pm0.003$ & 19.860$\pm0.002$ & 19.640$\pm0.003$ & 19.580$\pm0.003$ \\[-0.4ex]
30 & 21.438$\pm0.005$ & 21.385$\pm0.005$ & 21.399$\pm0.006$ & 21.340$\pm0.005$ & 21.211$\pm0.007$ & 21.184$\pm0.009$ \\[-0.4ex]
31 & 22.126$\pm0.005$ & 22.172$\pm0.005$ & 22.199$\pm0.006$ & 22.166$\pm0.005$ & 22.116$\pm0.007$ & 22.108$\pm0.011$ \\[-0.4ex]
32 & 21.449$\pm0.004$ & 21.374$\pm0.003$ & 21.357$\pm0.004$ & 21.308$\pm0.003$ & 21.226$\pm0.005$ & 21.197$\pm0.007$ \\[-0.4ex]


==> Table4_old.tex <==
05 &  9900$\pm200$ & 1.38$\pm0.05$  & $-0.15\pm0.10$ & $1.40\pm0.06$ & $-0.24\pm0.04$ & $0.00\pm0.01$ &      \nodata        & $21.62\pm0.07$ \\[-0.4ex] % 449
08 & 13500$\pm100$ & 2.10$\pm0.05$  & $-0.12\pm0.05$ & $1.58\pm0.05$ & $-0.87\pm0.02$ & $0.17\pm0.03$ & $6.00\pm0.60$ & $19.53\pm0.09$  \\[-0.4ex] % 229 ext
14 &  9300$\pm200$ & 1.27$\pm0.05$  & $-0.14\pm0.07$ & $1.40\pm0.18$ & $-0.14\pm0.05$ & $0.10\pm0.01$ & $6.10\pm0.65$ & $21.06\pm0.09$ \\[-0.4ex] % 396
16 & 12750$\pm300$ & 1.77$\pm0.05$  & $+0.02\pm0.08$ & $1.35\pm0.05$ & $-0.76\pm0.06$ & $0.10\pm0.02$ & $2.96\pm0.30$ & $20.45\pm0.07$  \\[-0.4ex] % 121
20 &  8150$\pm75 $ & 0.79$\pm0.05$  & $+0.01\pm0.05$ & $1.15\pm0.09$ & $+0.06\pm0.05$ & $0.28\pm0.05$ & $3.39\pm0.80$ & $20.36\pm0.20$  \\[-0.4ex] % 225
21 &  9150$\pm350$ & 1.41$\pm0.05$  & $-0.30\pm0.12$ & $1.56\pm0.11$ & $-0.10\pm0.07$ & $0.08\pm0.03$ & $4.38\pm2.00$ & $21.59\pm0.15$ \\[-0.4ex] % 630
23 &  8100$\pm50 $ & 0.83$\pm0.05$  & $-0.07\pm0.04$ & $1.20\pm0.08$ & $+0.08\pm0.03$ & $0.33\pm0.02$ & $3.39\pm0.25$ & $20.00\pm0.05$  \\[-0.4ex] % 173
26 &  7985$\pm25 $ & 0.75$\pm0.05$  & $-0.26\pm0.04$ & $1.14\pm0.07$ & $+0.07\pm0.02$ & $0.24\pm0.03$ & $2.17\pm0.60$ & $20.70\pm0.14$ \\[-0.4ex] % 140
29 &  8425$\pm25 $ & 0.87$\pm0.05$  & $+0.07\pm0.04$ & $1.17\pm0.06$ & $-0.01\pm0.03$ & $0.13\pm0.02$ & $5.50\pm0.60$ & $19.85\pm0.07$ \\[-0.4ex] % 061
31 & 11400$\pm200$ & 1.68$\pm0.05$  & $-0.10\pm0.07$ & $1.45\pm0.05$ & $-0.51\pm0.04$ & $0.02\pm0.01$ & $6.83\pm0.85$ & $21.46\pm0.07$  \\[-0.4ex] % 482
32 & 10950$\pm200$ & 1.74$\pm0.05$  & $-0.10\pm0.08$ & $1.58\pm0.06$ & $-0.40\pm0.04$  & $0.05\pm0.02$ & $6.09\pm0.50$ & $20.69\pm0.07$ \\[-0.4ex] % 159
33 & 10300$\pm100$ & 1.41$\pm0.05$  & $-0.05\pm0.06$ & $1.36\pm0.05$ & $-0.32\pm0.03$  & $0.06\pm0.03$ & $6.18\pm2.50$ & $21.17\pm0.13$ \\[-0.4ex] % 321
